Beyond Sentiment: A Multi-Agent Pipeline for Actionable Business Advice from Reviews

Customer reviews contain valuable signals about service quality, but converting large-scale review corpora into actionable business recommendations remains difficult. Standard sentiment/aspect analysis is largely descriptive, while direct prompting of large language models (LLMs) often yields generic and repetitive advice that is weakly grounded in user feedback. We propose a hierarchical decision-support pipeline that explicitly separates signal compression, problem abstraction, candidate generation, objective-based evaluation, and cost-aware routing into different agents. This architectural decomposition produces auditable intermediate artifacts and enables controllable trade-offs between advice quality and token budget. Experiments on Yelp reviews from three service domains show consistent improvements over single-pass LLM baselines across multiple advice quality dimensions, including actionability, relevance, and non-redundancy. A human evaluation further indicates that users generally prefer our system's recommendations. These results highlight the value of structured agentic decomposition for scalable, cost-aware business decision support.

==> acl-style-files-master/meta.tex <==

\subsection{Meta Agent}
%========================
% (Optional) Packages if you want the algorithm block:
% \usepackage{algorithm}
% \usepackage{algpseudocode}
%========================

% \subsection{Preference-Aware Meta-Agent Router}
\label{subsec:meta_router}

Our framework admits multiple \emph{configurations} that trade off output quality against
inference cost (tokens and latency). While the full multi-agent pipeline generally improves
robustness and structure, practitioners may prefer cheaper settings for interactive or
cost-sensitive deployments. We therefore introduce a \emph{meta-agent} (router) that selects
an execution configuration based on a user-specified quality--cost preference.

\paragraph{Configuration space.}
Let $x$ denote the input to the system (e.g., representative reviews and/or derived issues).
We define a discrete set of pipeline variants
$\mathcal{A}=\{A_0, A_{\neg I}, A_{\neg E}, A_{\neg I\neg E}, A_3\}$,
where $A_0$ is a single-pass baseline and the remaining variants correspond to enabling/disabling
agents (Issue Agent $I$ and Evaluation Agent $E$) in the pipeline.
The full framework is denoted by $A_3$ (Issue + Recommendation + Evaluation + Ranking).
In our experimental design, \emph{model-tier selection is applied only to the full framework}.
Accordingly, when $A_3$ is chosen we additionally select a model tier
$m \in \mathcal{M}$ (e.g., large/medium/Gemini), yielding the conditional configuration $(A_3,m)$.

\paragraph{Cost and quality signals.}
For a configuration $k$, we define a scalar \emph{cost} $C_k(x)$ and a scalar \emph{quality}
$Q_k(x)$. Cost may be defined as token usage, latency, or a combination:
\begin{equation}
C_k(x) \;=\; \lambda_{\mathrm{tok}}\;\mathrm{Tok}_k(x)\;+\;\lambda_{\mathrm{lat}}\;\mathrm{Lat}_k(x),
\label{eq:meta_cost}
\end{equation}
where $\mathrm{Tok}_k(x)$ is total input+output tokens across all LLM calls under $k$ and
$\mathrm{Lat}_k(x)$ is end-to-end wall-clock latency (both measurable at runtime).
Quality $Q_k(x)$ can be instantiated using (i) empirical expected quality from prior evaluation,
(ii) a lightweight predictor (learned router), or (iii) a small LLM judge; our formulation is agnostic.

To combine cost and quality in a single objective, we normalize both to $[0,1]$:
\begin{equation}
\widetilde{Q}_k(x)=\frac{Q_k(x)-Q_{\min}}{Q_{\max}-Q_{\min}},\quad
\widetilde{C}_k(x)=\frac{C_k(x)-C_{\min}}{C_{\max}-C_{\min}}.
\label{eq:meta_norm}
\end{equation}

\paragraph{User preference and routing objective.}
The user specifies a preference $p \in [0,1]$ controlling the emphasis on quality versus cost
($p=1$ prioritizes quality; $p=0$ prioritizes cost). We define the router utility:
\begin{equation}
U_k(x,p) \;=\; p\cdot \widetilde{Q}_k(x) \;-\; (1-p)\cdot \widetilde{C}_k(x).
\label{eq:meta_utility}
\end{equation}
The meta-agent selects the pipeline configuration that maximizes utility:
\begin{equation}
\begin{aligned}
a^{*}(x,p)=\arg\max_{a\in\mathcal{A}} U_a(x,p).
\label{eq:meta_select_pipeline}
\end{aligned}
\end{equation}
If $a^{*}(x,p)=A_3$, we additionally select the model tier:
\begin{equation}
m^{*}(x,p)=\arg\max_{m\in\mathcal{M}} U_{(A_3,m)}(x,p).
\label{eq:meta_select_tier}
\end{equation}
The executed configuration is $k^{*}(x,p)=a^{*}(x,p)$ if $a^{*}(x,p)\neq A_3$, and
$k^{*}(x,p)=(A_3,m^{*}(x,p))$ otherwise.

\paragraph{Scalar routing score.}
For interpretability and compatibility with a single control knob, we define the router score
$s \in [0,1]$ as
\begin{equation}
s := p,
\label{eq:meta_s_equals_p}
\end{equation}
so that increasing $s$ monotonically shifts the operating point from low-cost to high-quality.
When a step-function mapping from $s$ to discrete variants is required, the thresholds are derived
from configuration indifference points under the utility objective (Appendix~\ref{app:meta_thresholds}).

%------------------------
% Optional: include an algorithm block if you want.
%------------------------
\begin{algorithm}[t]
\caption{Preference-aware meta-agent routing}
\label{alg:meta_router}
\begin{algorithmic}[1]
\Require Input $x$, user preference $p\in[0,1]$, variants $\mathcal{A}$, tiers $\mathcal{M}$
\State Compute $s \gets p$
\For{$a \in \mathcal{A}$}
  \State Estimate/lookup $Q_a(x)$ and measure/estimate $C_a(x)$
  \State Compute $\widetilde{Q}_a(x), \widetilde{C}_a(x)$ using Eq.~\eqref{eq:meta_norm}
  \State $U_a \gets p\widetilde{Q}_a(x) - (1-p)\widetilde{C}_a(x)$
\EndFor
\State $a^\* \gets \arg\max_{a\in\mathcal{A}} U_a$
\If{$a^\* \neq A_3$}
  \State Execute $a^\*$ and return output
\Else
  \For{$m \in \mathcal{M}$}
    \State Estimate/lookup $Q_{(A_3,m)}(x)$ and measure/estimate $C_{(A_3,m)}(x)$
    \State Compute utility $U_{(A_3,m)}$ as in Eq.~\eqref{eq:meta_utility}
  \EndFor
  \State $m^\* \gets \arg\max_{m\in\mathcal{M}} U_{(A_3,m)}$
  \State Execute $(A_3,m^\*)$ and return output
\EndIf
\end{algorithmic}
\end{algorithm}

\section{Meta-Agent Routing Thresholds and Derivations}
\label{app:meta_thresholds}

This appendix derives the routing thresholds implied by the utility objective in
Eq.~\eqref{eq:meta_utility}, and describes a practical procedure for producing a
piecewise mapping from the scalar router score $s\in[0,1]$ to a discrete configuration.

\subsection{Indifference point between two configurations}
Consider two configurations $i$ and $j$ with normalized quality and cost
$(\widetilde{Q}_i,\widetilde{C}_i)$ and $(\widetilde{Q}_j,\widetilde{C}_j)$.
Using Eq.~\eqref{eq:meta_utility}, configuration $j$ is preferred to $i$ whenever
\begin{equation}
U_j(x,p) \ge U_i(x,p).
\end{equation}
The \emph{indifference point} $p^{*}$ between $i$ and $j$ is obtained by solving
$U_j(x,p^{*}) = U_i(x,p^{*})$:
\begin{align}
p^{*} \widetilde{Q}_j - (1-p^{*})\widetilde{C}_j
&= p^{*} \widetilde{Q}_i - (1-p^{*})\widetilde{C}_i \\
p^{*}(\widetilde{Q}_j-\widetilde{Q}_i) + p^{*}(\widetilde{C}_j-\widetilde{C}_i)
&= \widetilde{C}_j-\widetilde{C}_i.
\end{align}
Let $\Delta \widetilde{Q}=\widetilde{Q}_j-\widetilde{Q}_i$ and
$\Delta \widetilde{C}=\widetilde{C}_j-\widetilde{C}_i$. When $\Delta \widetilde{Q}+\Delta \widetilde{C} \neq 0$,
\begin{equation}
p^{*} \;=\; \frac{\Delta \widetilde{C}}{\Delta \widetilde{C}+\Delta \widetilde{Q}}.
\label{eq:meta_pstar}
\end{equation}
For $p < p^{*}$, configuration $i$ yields higher utility; for $p > p^{*}$, configuration $j$ yields higher utility.

\subsection{From indifference points to a piecewise mapping in $s$}
We set $s:=p$ (Eq.~\eqref{eq:meta_s_equals_p}). Let the candidate configurations be ordered by increasing
normalized cost, and remove dominated configurations (i.e., any configuration that has higher cost and
lower or equal quality than another). Denote the remaining Pareto-relevant configurations as
$k_0, k_1, \dots, k_K$ with $\widetilde{C}_{k_0}<\widetilde{C}_{k_1}<\dots<\widetilde{C}_{k_K}$.

For each adjacent pair $(k_{\ell},k_{\ell+1})$, compute the switch point $s^{*}_\ell$ using
Eq.~\eqref{eq:meta_pstar}. This yields thresholds:
\begin{equation}
0 = s^{*}_{-1} < s^{*}_0 < s^{*}_1 < \dots < s^{*}_{K-1} < s^{*}_{K}=1,
\end{equation}
and a piecewise mapping:
\begin{equation}
s \in [s^{*}_{\ell-1}, s^{*}_{\ell}) \;\Rightarrow\; k_\ell.
\label{eq:meta_piecewise}
\end{equation}
This procedure produces non-arbitrary bins: each threshold corresponds to the preference value at which
two neighboring Pareto-relevant configurations are equally optimal under the stated objective.

\subsection{Conditional thresholds for model-tier selection within the full framework}
When $A_3$ is selected, the same derivation applies within the tier set $\mathcal{M}$.
That is, we treat each tiered full-configuration $(A_3,m)$ as a candidate $k$ and compute
tier-specific switch points using Eq.~\eqref{eq:meta_pstar}, yielding a preference-conditioned
tier selection rule as in Eq.~\eqref{eq:meta_select_tier}.

\subsection{Practical instantiation with empirical measurements}
In the simplest instantiation, $Q_k(x)$ and $C_k(x)$ in Eq.~\eqref{eq:meta_norm} are replaced by empirical
expectations $\mathbb{E}[Q_k]$ and $\mathbb{E}[C_k]$ computed from validation runs for each configuration.
This enables offline computation of thresholds via Eq.~\eqref{eq:meta_pstar} and direct deployment at inference time.
More advanced instantiations can replace expected values with lightweight predictors $\widehat{Q}_k(x)$
to perform per-instance routing; the same objective and threshold analysis applies.



% =========================
% Meta-Agent Routing Module
% =========================
\subsection{Meta-Agent for Cost--Quality Adaptive Routing}
\label{sec:meta_agent}

A practical deployment constraint is that users vary in their tolerance for inference cost (token usage) versus their need for higher-quality recommendations. Our experiments already demonstrate (i) strong single-model baselines with substantial dependence on backbone choice (Table~1), and (ii) a cost--quality trade-off between model size/ensemble choices in the multi-agent scaffold (Section~6.3) \cite{turn0file0}. Motivated by this, we add a lightweight \emph{Meta-Agent} at the start of the pipeline that selects among a small set of pre-defined system configurations based on an explicit user preference.

\paragraph{Candidate configurations.}
We assume an ordered set of $K$ configurations $\mathcal{A}=\{A_0,\dots,A_{K-1}\}$ from cheapest to most expensive under a token-cost model. In our setting, we expose five pipeline levels:
\begin{itemize}
    \item $A_0$: Single-pass inference (no multi-agent scaffold).
    \item $A_1$: Multi-agent scaffold variant 1 (e.g., without Issue \& Evaluation).
    \item $A_2$: Multi-agent scaffold variant 2 (e.g., without Evaluation).
    \item $A_3$: Multi-agent scaffold variant 3 (e.g., without Issue).
    \item $A_4$: Full multi-agent scaffold.
\end{itemize}
We also support \emph{tiered backbones} within certain levels: for $A_0$ the user can choose among three single-model backbones (Llama, GPT-OSS, DeepSeek), consistent with the observed backbone sensitivity in vanilla baselines (Table~1) \cite{turn0file0}. Likewise, for $A_4$ we may select among model-size tiers (e.g., Three Big vs.\ Three Medium), consistent with the cost--quality discussion in Section~6.3 \cite{turn0file0}. (For clarity, we treat backbone selection as a nested decision after the pipeline level is chosen.)

\paragraph{Preference elicitation and scalarization.}
The user provides nonnegative weights $(w_Q,w_C)$ indicating emphasis on quality versus cost. We map this to a continuous \emph{quality emphasis} parameter:
\begin{equation}
\label{eq:pref_p}
p \;=\; \frac{w_Q}{w_Q+w_C} \in [0,1],
\end{equation}
where larger $p$ indicates a stronger preference for quality over cost. This follows a standard multi-objective scalarization approach: $(w_Q,w_C)$ expresses a trade-off, and $p$ is its normalized one-dimensional representation.

\paragraph{Cost-aware, near-uniform binning.}
A purely utility-optimal router can collapse to a small number of configurations when mean quality differences are small. In contrast, our goal is to offer \emph{interpretable, stable “gears”} that keep all $K$ options reachable while still reflecting that token costs are not evenly spaced (e.g., single-pass $\rightarrow$ multi-agent incurs a large multiplicative jump). Therefore, we introduce a monotone \emph{calibration layer} that maps $p$ into $K$ discrete bins using blended thresholds that are (i) close to uniform and (ii) mildly cost-aware.

Let $C_i$ denote the measured token cost of configuration $A_i$ (averaged over the dataset under a fixed evaluation setup), with $C_0 < C_1 < \cdots < C_{K-1}$. We define a normalized \emph{log-cost coordinate}:
\begin{equation}
\label{eq:logcost_g}
g_i \;=\; \frac{\log C_i - \log C_0}{\log C_{K-1} - \log C_0}\in[0,1], \qquad i=0,\dots,K-1.
\end{equation}
Log scaling is appropriate because token costs vary multiplicatively across configurations rather than additively.

Next, define cost-aware midpoints between adjacent options:
\begin{equation}
\label{eq:midpoints_m}
m_i \;=\; \frac{g_{i-1}+g_i}{2}, \qquad i=1,\dots,K-1,
\end{equation}
and uniform midpoints (exactly equal-width bins):
\begin{equation}
\label{eq:uniform_u}
u_i \;=\; \frac{i}{K}, \qquad i=1,\dots,K-1.
\end{equation}
Finally, we blend the two via a single hyperparameter $\varepsilon\in[0,1]$:
\begin{equation}
\label{eq:blend_b}
b_i(\varepsilon) \;=\; (1-\varepsilon)\,u_i \;+\; \varepsilon\,m_i, \qquad i=1,\dots,K-1.
\end{equation}
Here $\varepsilon=0$ yields exactly uniform bins; $\varepsilon=1$ yields purely cost-aware bins; intermediate values (e.g., $\varepsilon\in[0.2,0.4]$) provide near-uniform bins with modest cost adaptation.

\paragraph{Routing rule.}
Let $b_0=0$ and $b_K=1$. The Meta-Agent selects the configuration index:
\begin{equation}
\label{eq:routing_rule}
j \;=\; \sum_{i=1}^{K-1} \mathbf{1}\left[p \ge b_i(\varepsilon)\right],
\qquad
A \leftarrow A_j.
\end{equation}
This guarantees that each configuration $A_j$ corresponds to a non-empty interval $p\in[b_j,b_{j+1})$, ensuring full coverage.

\paragraph{Monotonicity and coverage (properties).}
Since $C_i$ is strictly increasing, $\log C_i$ and hence $g_i$ are strictly increasing. Therefore, $(m_i)_{i=1}^{K-1}$ is strictly increasing. The uniform thresholds $(u_i)$ are also strictly increasing; thus, for any $\varepsilon\in[0,1]$, $(b_i(\varepsilon))$ is strictly increasing as a convex combination of two increasing sequences. Consequently, the bins $[b_j,b_{j+1})$ partition $[0,1]$ into $K$ non-empty intervals, ensuring monotone routing and reachability of all options.

\paragraph{Concrete thresholds from token measurements (automotive example).}
Using our measured token costs for the five pipeline levels on the automotive dataset (tokens-only):
\[
(C_0,C_1,C_2,C_3,C_4)=(4822,\;30045,\;30166,\;71737,\;114441),
\]
we compute $g_i$ via Eq.~\eqref{eq:logcost_g}, midpoints $m_i$ via Eq.~\eqref{eq:midpoints_m}, and blended thresholds $b_i(\varepsilon)$ via Eq.~\eqref{eq:blend_b}. With $\varepsilon=0.3$, the resulting bin edges are:
\begin{equation}
\label{eq:thresholds_numeric}
\bigl(b_1,b_2,b_3,b_4\bigr) \approx (0.2267,\;0.4535,\;0.6347,\;0.8379).
\end{equation}
Thus, the five routing regions are:
\[
\begin{aligned}
p \in [0,0.2267) &\Rightarrow A_0, \\
p \in [0.2267,0.4535) &\Rightarrow A_1, \\
p \in [0.4535,0.6347) &\Rightarrow A_2, \\
p \in [0.6347,0.8379) &\Rightarrow A_3, \\
p \in [0.8379,1] &\Rightarrow A_4.
\end{aligned}
\]
These bins are close to uniform (nominally $0.2$ width) while reflecting the large multiplicative jump from $A_0$ to $A_1$ in token cost.

\paragraph{Nested backbone/tier selection.}
After selecting the pipeline level $A_j$, we optionally select a backbone tier when the configuration admits meaningful backbone variation. In particular:
\begin{itemize}
    \item If $A=A_0$, we select one of \{\texttt{Llama}, \texttt{DeepSeek}, \texttt{GPT-OSS}\} using a second application of the same binning rule over the three single-model costs (or a fixed mapping such as low-$p$ $\rightarrow$ cheapest backbone).
    \item If $A=A_4$, we select a multi-agent backbone tier (e.g., Three Medium vs.\ Three Big) using the same mechanism.
\end{itemize}
This hierarchical routing aligns with our empirical observations: single-model performance varies substantially across backbones (Table~1), whereas the multi-agent scaffold reduces variance and supports cost--quality trade-offs across model sizes (Section~6.3) \cite{turn0file0}. Moreover, ablation results indicate distinct contributions of the Issue and Evaluation agents, motivating exposure of intermediate configurations as user-selectable compute levels rather than forcing an all-or-nothing scaffold \cite{turn0file0}.

% =========================
% Meta-Agent Router Section
% =========================

\subsection{Meta-Agent Router: Preference-Guided System Selection}
\label{subsec:meta_router}

Our framework supports multiple inference configurations that trade off advice quality against computational cost (token usage).
To expose this trade-off to end users in an interpretable way, we introduce a lightweight \emph{Meta-Agent Router} that maps a
user preference (accuracy vs.\ cost) to one of a fixed set of pipeline configurations. The router is designed to (i) remain
multi-objective in principle, (ii) be monotone in the user preference, and (iii) keep \emph{all} configurations reachable
(i.e., avoid degenerate behavior where one option dominates due to dataset-level averages).

\paragraph{Candidate configurations.}
We assume a fixed, ordered set of $K{+}1$ pipeline configurations
$\mathcal{A} = \{A_0, A_1, \dots, A_K\}$ from cheapest to most expensive under token cost.
In our experiments, we use $K{=}4$ (five choices):
\begin{align*}
A_0 &: \text{Single-LLM (baseline)}\\
A_1 &: \text{Ablation: w/o Issue \& w/o Evaluation}\\
A_2 &: \text{Ablation: w/o Evaluation}\\
A_3 &: \text{Ablation: w/o Issue}\\
A_4 &: \text{Full multi-agent framework.}
\end{align*}
For each $A_i$ we record (from a calibration domain) its mean advice quality $Q_i$ and mean token cost $C_i$.

\paragraph{User preference as a multi-objective scalarization.}
The user specifies nonnegative weights $(w_Q,w_C)$ for quality vs.\ cost. We convert them into a single preference score:
\begin{equation}
p \;=\; \frac{w_Q}{w_Q+w_C} \in [0,1],
\label{eq:p_from_weights}
\end{equation}
where larger $p$ indicates stronger preference for quality (i.e., willingness to spend more tokens).

\paragraph{Why not direct utility maximization over mean $(Q_i,C_i)$?}
A standard approach is to select $\arg\max_i \big(p\widetilde{Q}_i - (1-p)\widetilde{C}_i\big)$ using normalized means.
However, in practice, dataset-level averages can make intermediate configurations appear dominated (e.g., similar quality but
higher token cost), collapsing the router to only one or two options. Since one goal of the router is to provide a stable
and interpretable ``compute knob'' (ensuring that each tier is selectable), we separate (a) the user preference modeling
(Eq.~\ref{eq:p_from_weights}) from (b) the discretization policy that maps $p$ to tiers.

\subsubsection{Cost--Quality Geometry and Near-Uniform Binning}
\label{subsec:bins}

We compute thresholds that are (i) \emph{near-uniform} in $p$ (for interpretability) while (ii) being \emph{aware} of the
empirical cost/quality spacing between configurations. The key idea is to build a one-dimensional progress coordinate over
configurations using both token cost and quality, then blend it with uniform thresholds.

\paragraph{Normalization.}
Let $C_i$ denote mean token cost and $Q_i$ mean quality for configuration $A_i$.
We normalize log-cost and quality to $[0,1]$:
\begin{align}
x_i &= \frac{\log C_i - \log C_0}{\log C_K - \log C_0}, \qquad x_i \in [0,1], \label{eq:log_cost_norm}\\
y_i &= \frac{Q_i - \min_j Q_j}{\max_j Q_j - \min_j Q_j}, \qquad y_i \in [0,1]. \label{eq:quality_norm}
\end{align}
We use $\log C_i$ because token costs are naturally multiplicative (large jumps between tiers), and log-scale yields additive
distances commonly used in systems-style analyses.

\paragraph{Quality+cost progress coordinate (arc-length).}
Define a polygonal chain over the ordered configurations in the $(x,y)$ plane, and compute cumulative arc-length:
\begin{equation}
s_0 = 0, \qquad
s_i = s_{i-1} + \sqrt{(x_i-x_{i-1})^2 + (y_i-y_{i-1})^2}\quad \text{for } i=1,\dots,K.
\label{eq:arc_length}
\end{equation}
Normalize to $[0,1]$:
\begin{equation}
S_i = \frac{s_i}{s_K}\in[0,1].
\label{eq:S_norm}
\end{equation}

\paragraph{Cost--quality midpoints.}
We compute midpoint thresholds between adjacent configurations in this progress coordinate:
\begin{equation}
m_i = \frac{S_{i-1}+S_i}{2}, \qquad i=1,\dots,K.
\label{eq:midpoints_m}
\end{equation}
If used directly, $\{m_i\}$ yields fully cost/quality-aware but potentially non-uniform bins in $p$.

\paragraph{Near-uniform blending.}
Uniform thresholds for $K{+}1$ choices are:
\begin{equation}
u_i = \frac{i}{K+1}, \qquad i=1,\dots,K.
\label{eq:uniform_thresholds}
\end{equation}
We define blended thresholds:
\begin{equation}
b_i(\varepsilon) = (1-\varepsilon)\,u_i + \varepsilon\,m_i, \qquad \varepsilon \in [0,1],
\label{eq:blended_thresholds}
\end{equation}
where $\varepsilon$ controls the trade-off:
$\varepsilon{=}0$ yields exactly uniform bins, and $\varepsilon{=}1$ yields fully cost/quality-aware bins.
In practice we set $\varepsilon \in [0.2,0.4]$ to obtain ``almost-uniform'' bins while respecting the empirical spacing.

\paragraph{Routing rule.}
Let $b_0=0$ and $b_{K+1}=1$. The router selects configuration index
\begin{equation}
j = \sum_{i=1}^{K} \mathbf{1}\!\left[p \ge b_i(\varepsilon)\right],
\qquad \text{and returns } A_j.
\label{eq:routing_rule}
\end{equation}
This rule is monotone in $p$ and guarantees all $K{+}1$ configurations are reachable.

\paragraph{Monotonicity and coverage (sketch).}
Since $\{u_i\}$ is strictly increasing and $\{m_i\}$ is strictly increasing when $C_0<\cdots<C_K$ and the configurations are ordered,
their convex combination $\{b_i(\varepsilon)\}$ is strictly increasing for any $\varepsilon\in[0,1]$. Therefore
$0=b_0<b_1<\cdots<b_K<b_{K+1}=1$ and each interval $[b_j,b_{j+1})$ has positive length, implying every $A_j$ is selected for some user preference.

\subsubsection{Automotive Calibration: Concrete Threshold Values}
\label{subsec:automotive_thresholds}

We compute thresholds once using the Automotive domain (tokens-only) and then apply them unchanged to other domains.
Table~\ref{tab:auto_cost_quality} lists the calibration statistics for the five configurations.

\begin{table}[t]
\centering
\small
\begin{tabular}{lrr}
\toprule
Configuration & Quality $Q_i$ & Tokens $C_i$ \\
\midrule
$A_0$ (Single LLM) & 93.1 & 4{,}822 \\
$A_1$ (w/o Issue \& Eval) & 95.2 & 30{,}045 \\
$A_2$ (w/o Eval) & 94.4 & 30{,}166 \\
$A_3$ (w/o Issue) & 95.0 & 71{,}737 \\
$A_4$ (Full) & 95.2 & 114{,}441 \\
\bottomrule
\end{tabular}
\caption{Automotive calibration statistics (mean quality and mean token cost) used to compute router thresholds.
We use tokens-only cost for binning.}
\label{tab:auto_cost_quality}
\end{table}

Using Eqs.~\ref{eq:log_cost_norm}--\ref{eq:midpoints_m}, the resulting midpoints in the cost--quality progress coordinate are:
\begin{equation}
m \approx [0.2741,\; 0.6385,\; 0.8228,\; 0.9583].
\label{eq:auto_midpoints}
\end{equation}
With $\varepsilon{=}0.3$ in Eq.~\ref{eq:blended_thresholds} (our default ``almost-uniform'' choice),
the blended thresholds are:
\begin{equation}
b(\varepsilon{=}0.3)\approx [0.2222,\; 0.4716,\; 0.6668,\; 0.8475].
\label{eq:auto_thresholds_eps03}
\end{equation}
Therefore, the final bins over $p$ are:
\begin{align*}
p \in [0,0.2222) &\Rightarrow A_0 \\
p \in [0.2222,0.4716) &\Rightarrow A_1 \\
p \in [0.4716,0.6668) &\Rightarrow A_2 \\
p \in [0.6668,0.8475) &\Rightarrow A_3 \\
p \in [0.8475,1] &\Rightarrow A_4.
\end{align*}

\paragraph{Is Automotive-only calibration acceptable?}
Yes, provided it is framed as \emph{threshold calibration on a development split}:
we calibrate thresholds once on Automotive and then \emph{freeze} them for evaluation on other domains.
This avoids per-domain tuning while keeping the router deterministic and reproducible.

\subsubsection{Nested Selection for Backbone Tiers (Single-LLM and Full Framework)}
\label{subsec:nested_tiers}

Some configurations admit meaningful backbone variation.
In particular, our single-LLM baseline supports three backbones (Llama, DeepSeek, GPT-OSS). When the router selects $A_0$, we apply the same binning mechanism
(Eqs.~\ref{eq:log_cost_norm}--\ref{eq:routing_rule}) over the three single-LLM options using their Automotive $(Q,C)$ statistics.
With $\varepsilon{=}0.3$, the resulting two thresholds are:
\begin{equation}
b^{(A_0)}(\varepsilon{=}0.3)\approx [0.3017,\; 0.6851],
\label{eq:single_llm_thresholds}
\end{equation}
yielding:
\begin{align*}
p \in [0,0.3017) &\Rightarrow \text{Llama},\\
p \in [0.3017,0.6851) &\Rightarrow \text{DeepSeek},\\
p \in [0.6851,1] &\Rightarrow \text{GPT-OSS}.
\end{align*}
Analogously, if the full framework admits multiple tiers (e.g., Big vs.\ Medium), we can apply the same nested routing procedure
using the corresponding $(Q,C)$ calibration values.

\subsubsection{Meta-Agent Router Algorithm}
\label{subsec:router_algorithm}

\begin{algorithm}[t]
\caption{Meta-Agent Router (tokens-only, near-uniform cost--quality bins)}
\label{alg:meta_router}
\small
\begin{algorithmic}[1]
\Require User weights $(w_Q,w_C)$; calibration stats $\{(Q_i,C_i)\}_{i=0}^{K}$; blend parameter $\varepsilon$
\State Compute preference $p \leftarrow \frac{w_Q}{w_Q+w_C}$ \Comment{Eq.~\ref{eq:p_from_weights}}
\State Compute $x_i$ and $y_i$ for all $i$ \Comment{Eqs.~\ref{eq:log_cost_norm}, \ref{eq:quality_norm}}
\State Compute $S_i$ via arc-length \Comment{Eqs.~\ref{eq:arc_length}, \ref{eq:S_norm}}
\State Compute midpoints $m_i \leftarrow (S_{i-1}+S_i)/2$ \Comment{Eq.~\ref{eq:midpoints_m}}
\State Compute thresholds $b_i(\varepsilon)\leftarrow (1-\varepsilon)\frac{i}{K+1}+\varepsilon m_i$ \Comment{Eq.~\ref{eq:blended_thresholds}}
\State Select $j \leftarrow \sum_{i=1}^{K}\mathbf{1}[p \ge b_i(\varepsilon)]$ \Comment{Eq.~\ref{eq:routing_rule}}
\State \Return Configuration $A_j$
\end{algorithmic}
\end{algorithm}



% --------------------------- Meta-Agent Routing (Paper-ready) ---------------------------
% --------------------------- Meta-Agent Routing (Paper-ready) ---------------------------
\subsection{Meta-Agent for Preference-Aware System Routing}
\label{sec:meta_agent}

Our framework can be instantiated with multiple configurations that trade off
(i) recommendation quality and (ii) inference cost. As discussed in our cost--quality analysis
(\S6.3) and ablation results (Appendix~C), different agentic components and backbone choices
yield comparable mean quality in some settings while incurring materially different token budgets.
To provide a simple and transparent deployment control, we introduce a \emph{meta-agent} that
routes each user request to an appropriate configuration based on a user-specified preference
between accuracy and cost. This meta-agent does not alter the underlying pipeline; instead, it
implements a lightweight \emph{preference-to-configuration} mapping that keeps all intended
compute tiers reachable and interpretable. \cite{ } % (Add relevant citations if needed.)

\paragraph{User preference score.}
The user specifies nonnegative weights $(w_Q, w_C)$ indicating relative emphasis on quality
and cost. We convert these into a single scalar preference
\begin{equation}
p \;=\; \frac{w_Q}{w_Q+w_C} \in [0,1],
\label{eq:pref_score}
\end{equation}
where larger $p$ indicates greater willingness to spend tokens to improve output quality.

\paragraph{Candidate configurations and token costs.}
Let $\{A_0,\dots,A_4\}$ denote an ordered set of five pipeline configurations from cheapest to
most expensive, with measured token costs $C_0 < C_1 < C_2 < C_3 < C_4$ (tokens-only).
Concretely, we use:
\begin{itemize}
    \item $A_0$: Single-LLM inference (one-prompt, no framework),
    \item $A_1$: Framework w/o Issue Agent and w/o Evaluation Agent,
    \item $A_2$: Framework w/o Evaluation Agent,
    \item $A_3$: Framework w/o Issue Agent,
    \item $A_4$: Full multi-agent framework (Issue + Recommendation + Evaluation + Ranking).
\end{itemize}
This ordering matches the incremental inclusion of agentic components observed in the ablation
study (Appendix~C) and is aligned with the pipeline structure (Figure~2).  % See main paper.

\paragraph{Motivation: why not use utility-optimal thresholds directly?}
A standard approach would select $A_j$ via an argmax of a scalarized utility
(e.g., $p\widetilde{Q}_j - (1-p)\widetilde{C}_j$). However, using mean quality scores alone can
cause intermediate configurations to become \emph{dominated} (never selected) when quality
differences are small relative to token costs. In practical deployments, teams often require
explicit, stable ``gears'' for budgeting, latency/cost envelopes, and operational policy
(including the ability to intentionally choose intermediate tiers). Therefore, we separate:
(i) preference elicitation (Eq.~\ref{eq:pref_score}) from (ii) a calibrated discretization that
ensures near-uniform coverage while still reflecting non-uniform token gaps.

\paragraph{Cost-aware uniformization via log-token geometry.}
Token costs are typically separated by multiplicative factors rather than additive increments.
We therefore define a normalized log-cost coordinate:
\begin{equation}
g_i \;=\; \frac{\log C_i - \log C_0}{\log C_4 - \log C_0},
\qquad i\in\{0,\dots,4\},
\label{eq:log_cost_coord}
\end{equation}
so that $g_0=0$ and $g_4=1$. Next, define cost-aware midpoints between adjacent configurations:
\begin{equation}
m_i \;=\; \frac{g_{i-1}+g_i}{2},
\qquad i\in\{1,\dots,4\}.
\label{eq:midpoints}
\end{equation}
If we used $\{m_i\}$ directly as thresholds, bins would be fully cost-aware but not uniform. For
a more interpretable control (approximately equal probability mass across the preference axis),
we blend these midpoints with uniform thresholds:
\begin{equation}
u_i \;=\; \frac{i}{5}\quad (i=1,\dots,4),
\qquad
b_i(\varepsilon) \;=\; (1-\varepsilon)u_i + \varepsilon m_i,
\qquad \varepsilon\in[0,1].
\label{eq:blended_thresholds}
\end{equation}
Here, $\varepsilon$ controls the trade-off between interpretability and cost-awareness:
$\varepsilon=0$ yields exactly uniform bins, while $\varepsilon=1$ yields purely cost-aware
(midpoint) bins. We use a small $\varepsilon$ (e.g., $0.2$--$0.4$) to obtain \emph{almost-uniform}
bins that still acknowledge large token jumps (notably from $A_0$ to $A_1$).

\paragraph{Routing rule.}
Let $b_0=0$ and $b_5=1$. The meta-agent selects the configuration index $j\in\{0,\dots,4\}$ by
\begin{equation}
j \;=\; \sum_{i=1}^{4} \mathbf{1}\!\left[p \ge b_i(\varepsilon)\right],
\qquad
A \leftarrow A_j,
\label{eq:routing_rule}
\end{equation}
which deterministically maps $p$ to exactly one of the five tiers.

\paragraph{Monotonicity and coverage.}
Assuming $C_0<\cdots<C_4$, the sequence $\{g_i\}$ is strictly increasing and so are the
midpoints $\{m_i\}$. Since $\{u_i\}$ is also strictly increasing, the blended thresholds
$\{b_i(\varepsilon)\}$ are strictly increasing for any $\varepsilon\in[0,1]$. Hence each interval
$[b_j, b_{j+1})$ has positive length, guaranteeing that every configuration $A_j$ is selected for
a non-empty range of $p$. This provides stable user control while remaining consistent with
token-cost geometry.

\paragraph{Example: token-only thresholds for the automotive setting.}
Using the measured token costs (tokens-only):
\begin{equation}
(C_0,C_1,C_2,C_3,C_4)
=
(4822,\;30045,\;30166,\;71737,\;114441),
\label{eq:example_costs}
\end{equation}
we compute $g_i$ from Eq.~\ref{eq:log_cost_coord}, then $m_i$ from Eq.~\ref{eq:midpoints}, and
finally the blended thresholds from Eq.~\ref{eq:blended_thresholds}. For $\varepsilon=0.3$,
this yields:
\begin{equation}
\left(b_1,b_2,b_3,b_4\right)
\approx
(0.2267,\;0.4535,\;0.6347,\;0.8379).
\label{eq:example_thresholds}
\end{equation}
Thus, the five routing bins are:
\begin{align}
p &\in [0,\,0.2267) &&\Rightarrow\; A_0 \quad \text{(Single LLM)}, \nonumber\\
p &\in [0.2267,\,0.4535) &&\Rightarrow\; A_1 \quad \text{(w/o Issue \& Eval)}, \nonumber\\
p &\in [0.4535,\,0.6347) &&\Rightarrow\; A_2 \quad \text{(w/o Eval)}, \nonumber\\
p &\in [0.6347,\,0.8379) &&\Rightarrow\; A_3 \quad \text{(w/o Issue)}, \nonumber\\
p &\in [0.8379,\,1] &&\Rightarrow\; A_4 \quad \text{(Full framework)}.
\label{eq:bins}
\end{align}

\paragraph{Backbone selection within tiers.}
Some tiers admit multiple backbone choices. In particular, $A_0$ (single-LLM inference) can use
any of $\{\textsc{Llama}, \textsc{GPT-OSS}, \textsc{DeepSeek}\}$, consistent with our single-model
baseline evaluation (Table~1). We implement backbone selection as a second-stage choice that is
invoked only when needed:
\begin{equation}
M =
\begin{cases}
\{\textsc{Llama}, \textsc{GPT-OSS}, \textsc{DeepSeek}\}, & \text{if } A=A_0,\\
\{\textsc{Big}, \textsc{Medium}\}, & \text{if } A=A_4 \text{ and multiple tiers are enabled},\\
\varnothing, & \text{otherwise.}
\end{cases}
\label{eq:conditional_backbone}
\end{equation}
In deployments that require a single deterministic backbone per tier, one may fix the backbone
(e.g., GPT-OSS for $A_0$) and retain only the pipeline-level routing of Eq.~\ref{eq:routing_rule}.

\paragraph{Discussion.}
The proposed meta-agent provides a simple interface for practitioners to trade off inference cost
and output quality while maintaining interpretable, stable compute tiers. By blending uniform and
cost-aware thresholds, the routing policy yields near-uniform preference bins yet respects the
fact that token budgets are not evenly spaced across pipeline variants. This design is particularly
useful in settings where mean quality differences between variants are modest (as observed in our
cost--quality results) but operational policies require explicit intermediate budget options.
% ---------------------------------------------------------------------------------------
\subsection{Meta Agent}
\label{sec:meta_agent}

Our framework can be instantiated with multiple configurations that trade off
(i) recommendation quality and (ii) inference cost. As discussed in our cost--quality analysis
(\S6.3) and ablation results (Appendix~C), different agentic components and backbone choices
yield comparable mean quality in some settings while incurring materially different token budgets.
To provide a simple and transparent deployment control, we introduce a \emph{meta-agent} that
routes each user request to an appropriate configuration based on a user-specified preference
between accuracy and cost. This meta-agent does not alter the underlying pipeline; instead, it
implements a lightweight \emph{preference-to-configuration} mapping that keeps all intended
compute tiers reachable and interpretable. \cite{ } % (Add relevant citations if needed.)

\paragraph{User preference score.}
The user specifies nonnegative weights $(w_Q, w_C)$ indicating relative emphasis on quality
and cost. We convert these into a single scalar preference
\begin{equation}
p \;=\; \frac{w_Q}{w_Q+w_C} \in [0,1],
\label{eq:pref_score}
\end{equation}
where larger $p$ indicates greater willingness to spend tokens to improve output quality.

\paragraph{Candidate configurations and token costs.}
Let $\{A_0,\dots,A_4\}$ denote an ordered set of five pipeline configurations from cheapest to
most expensive, with measured token costs $C_0 < C_1 < C_2 < C_3 < C_4$ (tokens-only).
Concretely, we use:
\begin{itemize}
    \item $A_0$: Single-LLM inference (one-prompt, no framework),
    \item $A_1$: Framework w/o Issue Agent and w/o Evaluation Agent,
    \item $A_2$: Framework w/o Evaluation Agent,
    \item $A_3$: Framework w/o Issue Agent,
    \item $A_4$: Full multi-agent framework (Issue + Recommendation + Evaluation + Ranking).
\end{itemize}
This ordering matches the incremental inclusion of agentic components observed in the ablation
study (Appendix~C) and is aligned with the pipeline structure (Figure~2).  % See main paper.

\paragraph{Motivation: why not use utility-optimal thresholds directly?}
A standard approach would select $A_j$ via an argmax of a scalarized utility
(e.g., $p\widetilde{Q}_j - (1-p)\widetilde{C}_j$). However, using mean quality scores alone can
cause intermediate configurations to become \emph{dominated} (never selected) when quality
differences are small relative to token costs. In practical deployments, teams often require
explicit, stable ``gears'' for budgeting, latency/cost envelopes, and operational policy
(including the ability to intentionally choose intermediate tiers). Therefore, we separate:
(i) preference elicitation (Eq.~\ref{eq:pref_score}) from (ii) a calibrated discretization that
ensures near-uniform coverage while still reflecting non-uniform token gaps.

\paragraph{Cost-aware uniformization via log-token geometry.}
Token costs are typically separated by multiplicative factors rather than additive increments.
We therefore define a normalized log-cost coordinate:
\begin{equation}
g_i \;=\; \frac{\log C_i - \log C_0}{\log C_4 - \log C_0},
\qquad i\in\{0,\dots,4\},
\label{eq:log_cost_coord}
\end{equation}
so that $g_0=0$ and $g_4=1$. Next, define cost-aware midpoints between adjacent configurations:
\begin{equation}
m_i \;=\; \frac{g_{i-1}+g_i}{2},
\qquad i\in\{1,\dots,4\}.
\label{eq:midpoints}
\end{equation}
If we used $\{m_i\}$ directly as thresholds, bins would be fully cost-aware but not uniform. For
a more interpretable control (approximately equal probability mass across the preference axis),
we blend these midpoints with uniform thresholds:
\begin{equation}
\begin{split}
u_i &= \frac{i}{5}, \quad i \in \{1,2,3,4\},\\
b_i(\varepsilon) &= (1-\varepsilon)\,u_i + \varepsilon\, m_i, \quad \varepsilon \in [0,1].
\end{split}
\label{eq:blended_thresholds}
\end{equation}

Here, $\varepsilon$ controls the trade-off between interpretability and cost-awareness:
$\varepsilon=0$ yields exactly uniform bins, while $\varepsilon=1$ yields purely cost-aware
(midpoint) bins. We use a small $\varepsilon$ (e.g., $0.2$--$0.4$) to obtain \emph{almost-uniform}
bins that still acknowledge large token jumps (notably from $A_0$ to $A_1$).

\paragraph{Routing rule.}
Let $b_0=0$ and $b_5=1$. The meta-agent selects the configuration index $j\in\{0,\dots,4\}$ by
\begin{equation}
j \;=\; \sum_{i=1}^{4} \mathbf{1}\!\left[p \ge b_i(\varepsilon)\right],
\qquad
A \leftarrow A_j,
\label{eq:routing_rule}
\end{equation}
which deterministically maps $p$ to exactly one of the five tiers.

\paragraph{Monotonicity and coverage.}
Assuming $C_0<\cdots<C_4$, the sequence $\{g_i\}$ is strictly increasing and so are the
midpoints $\{m_i\}$. Since $\{u_i\}$ is also strictly increasing, the blended thresholds
$\{b_i(\varepsilon)\}$ are strictly increasing for any $\varepsilon\in[0,1]$. Hence each interval
$[b_j, b_{j+1})$ has positive length, guaranteeing that every configuration $A_j$ is selected for
a non-empty range of $p$. This provides stable user control while remaining consistent with
token-cost geometry.

\paragraph{Example: token-only thresholds for the automotive setting.}
Using the measured token costs (tokens-only):
\begin{table}[ht!]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{c c c c c}
\toprule
$C_0$ & $C_1$ & $C_2$ & $C_3$ & $C_4$ \\
\midrule
4822 & 30045 & 30166 & 71737 & 114441 \\
\bottomrule
\end{tabular}
\caption{Token consumed for the five pipeline configurations for Automotive domain.}
\label{tab:example_costs}
\end{table}


We compute $g_i$ from Eq.~\ref{eq:log_cost_coord}, then $m_i$ from Eq.~\ref{eq:midpoints}, and
finally the blended thresholds from Eq.~\ref{eq:blended_thresholds}. For $\varepsilon=0.3$,
this yields:
\begin{equation}
\left(b_1,b_2,b_3,b_4\right)
\approx
(0.2267,\;0.4535,\;0.6347,\;0.8379).
\label{eq:example_thresholds}
\end{equation}
Thus, the five routing bins are:
\[
\begin{aligned}
p &\in [0,0.2267) &\Rightarrow A_0, \\
p &\in [0.2267,0.4535) &\Rightarrow A_1, \\
p &\in [0.4535,0.6347) &\Rightarrow A_2, \\
p &\in [0.6347,0.8379) &\Rightarrow A_3, \\
p &\in [0.8379,1] &\Rightarrow A_4.
\end{aligned}
\]
These bins are close to uniform (nominally $0.2$ width) while reflecting the large multiplicative jump from $A_0$ to $A_1$ in token cost.
\paragraph{Backbone selection within tiers.}
Some tiers admit multiple backbone choices. In particular, $A_0$ (single-LLM inference) can use
any of $\{\textsc{Llama}, \textsc{DeepSeek}\}$, consistent with our single-model
baseline evaluation (Table~1). We implement backbone selection as a second-stage choice that is
invoked only when needed:
\begin{equation}
M =
\begin{cases}
\{\textsc{Llama}, \textsc{DeepSeek}\}, & \text{if } A=A_0,\\
\{\textsc{Big}, \textsc{Medium}\}, & \text{if } A=A_4 \text{ and multiple tiers are enabled},\\
\varnothing, & \text{otherwise.}
\end{cases}
\label{eq:conditional_backbone}
\end{equation}
In deployments that require a single deterministic backbone per tier, one may fix the backbone
(e.g., GPT-OSS for $A_0$) and retain only the pipeline-level routing of Eq.~\ref{eq:routing_rule}.

\paragraph{Discussion.}
The proposed meta-agent provides a simple interface for practitioners to trade off inference cost
and output quality while maintaining interpretable, stable compute tiers. By blending uniform and
cost-aware thresholds, the routing policy yields near-uniform preference bins yet respects the
fact that token budgets are not evenly spaced across pipeline variants. This design is particularly
useful in settings where mean quality differences between variants are modest (as observed in our
cost--quality results) but operational policies require explicit intermediate budget options.
% ---------------------------------------------------------------------------------------




==> acl-style-files-master/notes.tex <==
Add $\eta$ justification, experiments etc.
Add future work(RAG for policy, )
Human Evaluation, correlation etc
update figure fonts
add token and latency accounting per approach


Remove gpt oss 120 b single model results 

==> data-description.tex <==
\begin{table}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.15}
\caption{Automotive (\textit{Payless Parking and Car Rental}) Dataset}
\begin{tabular}{@{}p{0.7cm}|p{3.2cm}|p{3.0cm}|p{7.6cm}@{}}
\toprule
S.N. & Issue & Theme & Advice \\
\midrule
1 & Extra gas charges & Pricing \& Billing Issues &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a transparent gas charge calculation system on invoices\\
\textbullet\ Introduce a tiered pricing structure with clear gas charge thresholds\\
\textbullet\ Offer a gas charge estimator tool on the company website\\
\textbullet\ Provide a gas charge waiver option for customers who meet certain\\ criteria
\end{tabular}
\\
\midrule
2 & Failure to resolve complaints or provide callbacks & Customer Service Failures &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a Complaint Resolution Tracker to monitor and follow\\ up on customer complaints.\\
\textbullet\ Introduce a Callback Guarantee, ensuring customers receive a response\\ within a specified timeframe.\\
\textbullet\ Develop a Customer Service Escalation Procedure to quickly address\\ and resolve complex issues.\\
\textbullet\ Provide Ongoing Training for Customer Service Representatives on\\ effective communication and issue resolution skills.
\end{tabular}
\\
\midrule
3 & Interior was filthy & Vehicle Condition &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a mandatory vehicle inspection and cleaning protocol\\ before each rental.\\
\textbullet\ Provide customers with a vehicle condition report to sign off on at\\ the start of the rental period.\\
\textbullet\ Train staff on the importance of maintaining clean vehicles and\\ establish a system for reporting and addressing dirty vehicles.\\
\textbullet\ Offer a premium cleaning service for an additional fee to customers\\ who want an extra level of cleanliness.
\end{tabular}
\\
\midrule
4 & Long wait for shuttle & Shuttle \& Pickup Issues &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a real-time shuttle tracking system to provide customers\\ with accurate estimated arrival times.\\
\textbullet\ Increase the frequency of shuttle runs during peak hours to reduce\\ wait times.\\
\textbullet\ Designate specific pickup points with clear signage and seating\\ areas to improve the overall waiting experience.\\
\textbullet\ Offer a mobile app for customers to request pickups and receive\\ updates on shuttle schedules and delays.
\end{tabular}
\\
\midrule
5 & Misrepresentation of prices & Transparency \& Misrepresentation &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a clear and consistent pricing policy across all sales\\ channels.\\
\textbullet\ Provide detailed breakdowns of costs and fees associated with each\\ product or service.\\
\textbullet\ Introduce a price match guarantee to ensure customers are not\\ overcharged.\\
\textbullet\ Conduct regular audits to detect and prevent \\misrepresentation of prices by sales representatives or partners.
\end{tabular}
\\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.15}
\caption{Restaurant (\textit{New Orleans Creole Cookery}) Dataset}
\begin{tabular}{@{}p{0.7cm}|p{3.2cm}|p{3.0cm}|p{7.6cm}@{}}
\toprule
S.N. & Issue & Theme & Advice \\
\midrule
1 & Food served cold, stale, or not fresh & Food Quality &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a First-In-First-Out inventory system to ensure older\\ products are sold or used before newer ones.\\
\textbullet\ Conduct regular temperature checks on storage and display equipment\\ to prevent food from being stored at incorrect temperatures.\\
\textbullet\ Introduce a quality control checklist for kitchen staff to verify\\ the freshness and temperature of food before serving.\\
\textbullet\ Establish a supplier evaluation and rating system to ensure that\\ only high-quality, fresh ingredients are sourced.
\end{tabular}
\\
\midrule
2 & Rude and unprofessional staff behavior & Service \& Staff &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a comprehensive customer service training program for\\ all staff members.\\
\textbullet\ Develop a clear code of conduct and disciplinary policy for \\unprofessional behavior.\\
\textbullet\ Introduce a staff evaluation and feedback system to monitor and\\ address rude behavior.\\
\textbullet\ Hire a dedicated customer service manager to oversee staff \\interactions and provide coaching.
\end{tabular}
\\
\midrule
3 & Reservation not honored or lost & Reservation \& Wait Times &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a digital reservation system with automated confirmations\\ and reminders.\\
\textbullet\ Train staff to thoroughly verify reservations upon arrival and\\ have a clear protocol for handling lost or misplaced reservations.\\
\textbullet\ Offer a waitlist management system that provides real-time updates\\ to customers on wait times and reservation status.\\
\textbullet\ Establish a clear escalation procedure for customers whose reservations\\ are not honored, including a dedicated customer service \\contact and potential compensation or priority seating on the next\\ available table.
\end{tabular}
\\
\midrule
4 & Mandatory 20\% service fee deemed excessive & Pricing \& Billing &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Introduce a tiered service fee structure with varying percentages\\ based on the total bill amount.\\
\textbullet\ Offer an optional service fee waiver for loyal customers or those\\ who meet certain spending thresholds.\\
\textbullet\ Implement a transparent pricing model that clearly breaks down\\ the service fee and other charges.\\
\textbullet\ Consider reducing the mandatory service fee to 15\% and introduce\\ additional revenue streams through premium services.
\end{tabular}
\\
\midrule
5 & Lack of proper cooking & Kitchen Operations &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a standardized cooking time and temperature control\\ system for all menu items.\\
\textbullet\ Provide ongoing training and certification programs for kitchen\\ staff on proper cooking techniques.\\
\textbullet\ Introduce a quality control checklist to ensure dishes meet culinary\\ standards before being served.\\
\textbullet\ Invest in kitchen equipment upgrades, such as precision thermometers\\ and cookers, to improve cooking consistency.
\end{tabular}
\\
\bottomrule
\end{tabular}
\end{table}



\begin{table}[ht]
\centering
\small
\renewcommand{\arraystretch}{1.15}
\caption{Hospitality (\textit{Circus Circus Reno}) Dataset}
\begin{tabular}{@{}p{0.7cm}|p{3.2cm}|p{3.0cm}|p{7.6cm}@{}}
\toprule
S.N. & Issue & Theme & Advice \\
\midrule
1 & Delayed check-in process (up to 3 hours) & Check-in \& Reservation &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a digital check-in system to reduce wait times and\\ allow guests to complete the check-in process online before arrival.\\
\textbullet\ Increase front desk staffing during peak hours to handle a higher\\ volume of check-ins and reduce delays.\\
\textbullet\ Introduce a mobile check-in app that enables guests to check-in\\ remotely and receive a digital key, bypassing the need to wait in \\line at the front desk.\\
\textbullet\ Offer a priority check-in service for loyalty program members or\\ guests who have paid for an upgraded experience to minimize their \\wait time.
\end{tabular}
\\
\midrule
2 & Unclean rooms with hair, snot, and general dirt & Cleanliness \& Maintenance &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a rigorous room inspection checklist for housekeeping\\ staff to ensure thorough cleaning of all areas.\\
\textbullet\ Increase the frequency of deep cleaning and sanitization of \\high-touch areas and surfaces.\\
\textbullet\ Provide ongoing training and feedback to housekeeping staff on\\ proper cleaning techniques and protocols.\\
\textbullet\ Install a quality control process to monitor and address guest\\ complaints regarding room cleanliness.
\end{tabular}
\\
\midrule
3 & Excessive noise from stairwell late at night & Noise \& Room Location &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Install soundproofing materials in the stairwell and adjacent rooms.\\
\textbullet\ Implement quiet hours policy with increased security patrols during\\ late nights.\\
\textbullet\ Relocate rooms affected by stairwell noise to quieter areas of the\\ building.\\
\textbullet\ Install noise-reducing doors and seals on rooms near the stairwell.
\end{tabular}
\\
\midrule
4 & Dismissive response to complaints & Staff Attitude \& Service &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Implement a comprehensive customer complaint handling training\\ program for all staff members.\\
\textbullet\ Introduce a mystery shopping initiative to monitor staff attitude\\ and service quality.\\
\textbullet\ Develop a clear and transparent complaint escalation procedure\\ to ensure timely resolution.\\
\textbullet\ Conduct regular staff feedback sessions to identify and address\\ underlying issues contributing to dismissive responses.
\end{tabular}
\\
\midrule
5 & Lack of crowd and excitement at gaming tables & Experience &
\begin{tabular}[t]{@{}l@{}}
\textbullet\ Introduce themed nights and events to attract a specific crowd\\ and create a lively atmosphere.\\
\textbullet\ Implement a rewards program that incentivizes players to visit\\ and play at the gaming tables during off-peak hours.\\
\textbullet\ Offer interactive games and tournaments that allow players to \\compete against each other and create a sense of community.\\
\textbullet\ Hire energetic and charismatic dealers to create a more engaging\\ and entertaining experience at the gaming tables.
\end{tabular}
\\
\bottomrule
\end{tabular}
\end{table}


==> meta.tex <==

\subsection{Meta Agent}
%========================
% (Optional) Packages if you want the algorithm block:
% \usepackage{algorithm}
% \usepackage{algpseudocode}
%========================

% \subsection{Preference-Aware Meta-Agent Router}
\label{subsec:meta_router}

Our framework admits multiple \emph{configurations} that trade off output quality against
inference cost (tokens and latency). While the full multi-agent pipeline generally improves
robustness and structure, practitioners may prefer cheaper settings for interactive or
cost-sensitive deployments. We therefore introduce a \emph{meta-agent} (router) that selects
an execution configuration based on a user-specified quality--cost preference.

\paragraph{Configuration space.}
Let $x$ denote the input to the system (e.g., representative reviews and/or derived issues).
We define a discrete set of pipeline variants
$\mathcal{A}=\{A_0, A_{\neg I}, A_{\neg E}, A_{\neg I\neg E}, A_3\}$,
where $A_0$ is a single-pass baseline and the remaining variants correspond to enabling/disabling
agents (Issue Agent $I$ and Evaluation Agent $E$) in the pipeline.
The full framework is denoted by $A_3$ (Issue + Recommendation + Evaluation + Ranking).
In our experimental design, \emph{model-tier selection is applied only to the full framework}.
Accordingly, when $A_3$ is chosen we additionally select a model tier
$m \in \mathcal{M}$ (e.g., large/medium/Gemini), yielding the conditional configuration $(A_3,m)$.

\paragraph{Cost and quality signals.}
For a configuration $k$, we define a scalar \emph{cost} $C_k(x)$ and a scalar \emph{quality}
$Q_k(x)$. Cost may be defined as token usage, latency, or a combination:
\begin{equation}
C_k(x) \;=\; \lambda_{\mathrm{tok}}\;\mathrm{Tok}_k(x)\;+\;\lambda_{\mathrm{lat}}\;\mathrm{Lat}_k(x),
\label{eq:meta_cost}
\end{equation}
where $\mathrm{Tok}_k(x)$ is total input+output tokens across all LLM calls under $k$ and
$\mathrm{Lat}_k(x)$ is end-to-end wall-clock latency (both measurable at runtime).
Quality $Q_k(x)$ can be instantiated using (i) empirical expected quality from prior evaluation,
(ii) a lightweight predictor (learned router), or (iii) a small LLM judge; our formulation is agnostic.

To combine cost and quality in a single objective, we normalize both to $[0,1]$:
\begin{equation}
\widetilde{Q}_k(x)=\frac{Q_k(x)-Q_{\min}}{Q_{\max}-Q_{\min}},\quad
\widetilde{C}_k(x)=\frac{C_k(x)-C_{\min}}{C_{\max}-C_{\min}}.
\label{eq:meta_norm}
\end{equation}

\paragraph{User preference and routing objective.}
The user specifies a preference $p \in [0,1]$ controlling the emphasis on quality versus cost
($p=1$ prioritizes quality; $p=0$ prioritizes cost). We define the router utility:
\begin{equation}
U_k(x,p) \;=\; p\cdot \widetilde{Q}_k(x) \;-\; (1-p)\cdot \widetilde{C}_k(x).
\label{eq:meta_utility}
\end{equation}
The meta-agent selects the pipeline configuration that maximizes utility:
\begin{equation}
\begin{aligned}
a^{*}(x,p)=\arg\max_{a\in\mathcal{A}} U_a(x,p).
\label{eq:meta_select_pipeline}
\end{aligned}
\end{equation}
If $a^{*}(x,p)=A_3$, we additionally select the model tier:
\begin{equation}
m^{*}(x,p)=\arg\max_{m\in\mathcal{M}} U_{(A_3,m)}(x,p).
\label{eq:meta_select_tier}
\end{equation}
The executed configuration is $k^{*}(x,p)=a^{*}(x,p)$ if $a^{*}(x,p)\neq A_3$, and
$k^{*}(x,p)=(A_3,m^{*}(x,p))$ otherwise.

\paragraph{Scalar routing score.}
For interpretability and compatibility with a single control knob, we define the router score
$s \in [0,1]$ as
\begin{equation}
s := p,
\label{eq:meta_s_equals_p}
\end{equation}
so that increasing $s$ monotonically shifts the operating point from low-cost to high-quality.
When a step-function mapping from $s$ to discrete variants is required, the thresholds are derived
from configuration indifference points under the utility objective (Appendix~\ref{app:meta_thresholds}).

%------------------------
% Optional: include an algorithm block if you want.
%------------------------
\begin{algorithm}[t]
\caption{Preference-aware meta-agent routing}
\label{alg:meta_router}
\begin{algorithmic}[1]
\Require Input $x$, user preference $p\in[0,1]$, variants $\mathcal{A}$, tiers $\mathcal{M}$
\State Compute $s \gets p$
\For{$a \in \mathcal{A}$}
  \State Estimate/lookup $Q_a(x)$ and measure/estimate $C_a(x)$
  \State Compute $\widetilde{Q}_a(x), \widetilde{C}_a(x)$ using Eq.~\eqref{eq:meta_norm}
  \State $U_a \gets p\widetilde{Q}_a(x) - (1-p)\widetilde{C}_a(x)$
\EndFor
\State $a^\* \gets \arg\max_{a\in\mathcal{A}} U_a$
\If{$a^\* \neq A_3$}
  \State Execute $a^\*$ and return output
\Else
  \For{$m \in \mathcal{M}$}
    \State Estimate/lookup $Q_{(A_3,m)}(x)$ and measure/estimate $C_{(A_3,m)}(x)$
    \State Compute utility $U_{(A_3,m)}$ as in Eq.~\eqref{eq:meta_utility}
  \EndFor
  \State $m^\* \gets \arg\max_{m\in\mathcal{M}} U_{(A_3,m)}$
  \State Execute $(A_3,m^\*)$ and return output
\EndIf
\end{algorithmic}
\end{algorithm}

\section{Meta-Agent Routing Thresholds and Derivations}
\label{app:meta_thresholds}

This appendix derives the routing thresholds implied by the utility objective in
Eq.~\eqref{eq:meta_utility}, and describes a practical procedure for producing a
piecewise mapping from the scalar router score $s\in[0,1]$ to a discrete configuration.

\subsection{Indifference point between two configurations}
Consider two configurations $i$ and $j$ with normalized quality and cost
$(\widetilde{Q}_i,\widetilde{C}_i)$ and $(\widetilde{Q}_j,\widetilde{C}_j)$.
Using Eq.~\eqref{eq:meta_utility}, configuration $j$ is preferred to $i$ whenever
\begin{equation}
U_j(x,p) \ge U_i(x,p).
\end{equation}
The \emph{indifference point} $p^{*}$ between $i$ and $j$ is obtained by solving
$U_j(x,p^{*}) = U_i(x,p^{*})$:
\begin{align}
p^{*} \widetilde{Q}_j - (1-p^{*})\widetilde{C}_j
&= p^{*} \widetilde{Q}_i - (1-p^{*})\widetilde{C}_i \\
p^{*}(\widetilde{Q}_j-\widetilde{Q}_i) + p^{*}(\widetilde{C}_j-\widetilde{C}_i)
&= \widetilde{C}_j-\widetilde{C}_i.
\end{align}
Let $\Delta \widetilde{Q}=\widetilde{Q}_j-\widetilde{Q}_i$ and
$\Delta \widetilde{C}=\widetilde{C}_j-\widetilde{C}_i$. When $\Delta \widetilde{Q}+\Delta \widetilde{C} \neq 0$,
\begin{equation}
p^{*} \;=\; \frac{\Delta \widetilde{C}}{\Delta \widetilde{C}+\Delta \widetilde{Q}}.
\label{eq:meta_pstar}
\end{equation}
For $p < p^{*}$, configuration $i$ yields higher utility; for $p > p^{*}$, configuration $j$ yields higher utility.

\subsection{From indifference points to a piecewise mapping in $s$}
We set $s:=p$ (Eq.~\eqref{eq:meta_s_equals_p}). Let the candidate configurations be ordered by increasing
normalized cost, and remove dominated configurations (i.e., any configuration that has higher cost and
lower or equal quality than another). Denote the remaining Pareto-relevant configurations as
$k_0, k_1, \dots, k_K$ with $\widetilde{C}_{k_0}<\widetilde{C}_{k_1}<\dots<\widetilde{C}_{k_K}$.

For each adjacent pair $(k_{\ell},k_{\ell+1})$, compute the switch point $s^{*}_\ell$ using
Eq.~\eqref{eq:meta_pstar}. This yields thresholds:
\begin{equation}
0 = s^{*}_{-1} < s^{*}_0 < s^{*}_1 < \dots < s^{*}_{K-1} < s^{*}_{K}=1,
\end{equation}
and a piecewise mapping:
\begin{equation}
s \in [s^{*}_{\ell-1}, s^{*}_{\ell}) \;\Rightarrow\; k_\ell.
\label{eq:meta_piecewise}
\end{equation}
This procedure produces non-arbitrary bins: each threshold corresponds to the preference value at which
two neighboring Pareto-relevant configurations are equally optimal under the stated objective.

\subsection{Conditional thresholds for model-tier selection within the full framework}
When $A_3$ is selected, the same derivation applies within the tier set $\mathcal{M}$.
That is, we treat each tiered full-configuration $(A_3,m)$ as a candidate $k$ and compute
tier-specific switch points using Eq.~\eqref{eq:meta_pstar}, yielding a preference-conditioned
tier selection rule as in Eq.~\eqref{eq:meta_select_tier}.

\subsection{Practical instantiation with empirical measurements}
In the simplest instantiation, $Q_k(x)$ and $C_k(x)$ in Eq.~\eqref{eq:meta_norm} are replaced by empirical
expectations $\mathbb{E}[Q_k]$ and $\mathbb{E}[C_k]$ computed from validation runs for each configuration.
This enables offline computation of thresholds via Eq.~\eqref{eq:meta_pstar} and direct deployment at inference time.
More advanced instantiations can replace expected values with lightweight predictors $\widehat{Q}_k(x)$
to perform per-instance routing; the same objective and threshold analysis applies.



% =========================
% Meta-Agent Routing Module
% =========================
\subsection{Meta-Agent for Cost--Quality Adaptive Routing}
\label{sec:meta_agent}

A practical deployment constraint is that users vary in their tolerance for inference cost (token usage) versus their need for higher-quality recommendations. Our experiments already demonstrate (i) strong single-model baselines with substantial dependence on backbone choice (Table~1), and (ii) a cost--quality trade-off between model size/ensemble choices in the multi-agent scaffold (Section~6.3) \cite{turn0file0}. Motivated by this, we add a lightweight \emph{Meta-Agent} at the start of the pipeline that selects among a small set of pre-defined system configurations based on an explicit user preference.

\paragraph{Candidate configurations.}
We assume an ordered set of $K$ configurations $\mathcal{A}=\{A_0,\dots,A_{K-1}\}$ from cheapest to most expensive under a token-cost model. In our setting, we expose five pipeline levels:
\begin{itemize}
    \item $A_0$: Single-pass inference (no multi-agent scaffold).
    \item $A_1$: Multi-agent scaffold variant 1 (e.g., without Issue \& Evaluation).
    \item $A_2$: Multi-agent scaffold variant 2 (e.g., without Evaluation).
    \item $A_3$: Multi-agent scaffold variant 3 (e.g., without Issue).
    \item $A_4$: Full multi-agent scaffold.
\end{itemize}
We also support \emph{tiered backbones} within certain levels: for $A_0$ the user can choose among three single-model backbones (Llama, GPT-OSS, DeepSeek), consistent with the observed backbone sensitivity in vanilla baselines (Table~1) \cite{turn0file0}. Likewise, for $A_4$ we may select among model-size tiers (e.g., Three Big vs.\ Three Medium), consistent with the cost--quality discussion in Section~6.3 \cite{turn0file0}. (For clarity, we treat backbone selection as a nested decision after the pipeline level is chosen.)

\paragraph{Preference elicitation and scalarization.}
The user provides nonnegative weights $(w_Q,w_C)$ indicating emphasis on quality versus cost. We map this to a continuous \emph{quality emphasis} parameter:
\begin{equation}
\label{eq:pref_p}
p \;=\; \frac{w_Q}{w_Q+w_C} \in [0,1],
\end{equation}
where larger $p$ indicates a stronger preference for quality over cost. This follows a standard multi-objective scalarization approach: $(w_Q,w_C)$ expresses a trade-off, and $p$ is its normalized one-dimensional representation.

\paragraph{Cost-aware, near-uniform binning.}
A purely utility-optimal router can collapse to a small number of configurations when mean quality differences are small. In contrast, our goal is to offer \emph{interpretable, stable “gears”} that keep all $K$ options reachable while still reflecting that token costs are not evenly spaced (e.g., single-pass $\rightarrow$ multi-agent incurs a large multiplicative jump). Therefore, we introduce a monotone \emph{calibration layer} that maps $p$ into $K$ discrete bins using blended thresholds that are (i) close to uniform and (ii) mildly cost-aware.

Let $C_i$ denote the measured token cost of configuration $A_i$ (averaged over the dataset under a fixed evaluation setup), with $C_0 < C_1 < \cdots < C_{K-1}$. We define a normalized \emph{log-cost coordinate}:
\begin{equation}
\label{eq:logcost_g}
g_i \;=\; \frac{\log C_i - \log C_0}{\log C_{K-1} - \log C_0}\in[0,1], \qquad i=0,\dots,K-1.
\end{equation}
Log scaling is appropriate because token costs vary multiplicatively across configurations rather than additively.

Next, define cost-aware midpoints between adjacent options:
\begin{equation}
\label{eq:midpoints_m}
m_i \;=\; \frac{g_{i-1}+g_i}{2}, \qquad i=1,\dots,K-1,
\end{equation}
and uniform midpoints (exactly equal-width bins):
\begin{equation}
\label{eq:uniform_u}
u_i \;=\; \frac{i}{K}, \qquad i=1,\dots,K-1.
\end{equation}
Finally, we blend the two via a single hyperparameter $\varepsilon\in[0,1]$:
\begin{equation}
\label{eq:blend_b}
b_i(\varepsilon) \;=\; (1-\varepsilon)\,u_i \;+\; \varepsilon\,m_i, \qquad i=1,\dots,K-1.
\end{equation}
Here $\varepsilon=0$ yields exactly uniform bins; $\varepsilon=1$ yields purely cost-aware bins; intermediate values (e.g., $\varepsilon\in[0.2,0.4]$) provide near-uniform bins with modest cost adaptation.

\paragraph{Routing rule.}
Let $b_0=0$ and $b_K=1$. The Meta-Agent selects the configuration index:
\begin{equation}
\label{eq:routing_rule}
j \;=\; \sum_{i=1}^{K-1} \mathbf{1}\left[p \ge b_i(\varepsilon)\right],
\qquad
A \leftarrow A_j.
\end{equation}
This guarantees that each configuration $A_j$ corresponds to a non-empty interval $p\in[b_j,b_{j+1})$, ensuring full coverage.

\paragraph{Monotonicity and coverage (properties).}
Since $C_i$ is strictly increasing, $\log C_i$ and hence $g_i$ are strictly increasing. Therefore, $(m_i)_{i=1}^{K-1}$ is strictly increasing. The uniform thresholds $(u_i)$ are also strictly increasing; thus, for any $\varepsilon\in[0,1]$, $(b_i(\varepsilon))$ is strictly increasing as a convex combination of two increasing sequences. Consequently, the bins $[b_j,b_{j+1})$ partition $[0,1]$ into $K$ non-empty intervals, ensuring monotone routing and reachability of all options.

\paragraph{Concrete thresholds from token measurements (automotive example).}
Using our measured token costs for the five pipeline levels on the automotive dataset (tokens-only):
\[
(C_0,C_1,C_2,C_3,C_4)=(4822,\;30045,\;30166,\;71737,\;114441),
\]
we compute $g_i$ via Eq.~\eqref{eq:logcost_g}, midpoints $m_i$ via Eq.~\eqref{eq:midpoints_m}, and blended thresholds $b_i(\varepsilon)$ via Eq.~\eqref{eq:blend_b}. With $\varepsilon=0.3$, the resulting bin edges are:
\begin{equation}
\label{eq:thresholds_numeric}
\bigl(b_1,b_2,b_3,b_4\bigr) \approx (0.2267,\;0.4535,\;0.6347,\;0.8379).
\end{equation}
Thus, the five routing regions are:
\[
\begin{aligned}
p \in [0,0.2267) &\Rightarrow A_0, \\
p \in [0.2267,0.4535) &\Rightarrow A_1, \\
p \in [0.4535,0.6347) &\Rightarrow A_2, \\
p \in [0.6347,0.8379) &\Rightarrow A_3, \\
p \in [0.8379,1] &\Rightarrow A_4.
\end{aligned}
\]
These bins are close to uniform (nominally $0.2$ width) while reflecting the large multiplicative jump from $A_0$ to $A_1$ in token cost.

\paragraph{Nested backbone/tier selection.}
After selecting the pipeline level $A_j$, we optionally select a backbone tier when the configuration admits meaningful backbone variation. In particular:
\begin{itemize}
    \item If $A=A_0$, we select one of \{\texttt{Llama}, \texttt{DeepSeek}, \texttt{GPT-OSS}\} using a second application of the same binning rule over the three single-model costs (or a fixed mapping such as low-$p$ $\rightarrow$ cheapest backbone).
    \item If $A=A_4$, we select a multi-agent backbone tier (e.g., Three Medium vs.\ Three Big) using the same mechanism.
\end{itemize}
This hierarchical routing aligns with our empirical observations: single-model performance varies substantially across backbones (Table~1), whereas the multi-agent scaffold reduces variance and supports cost--quality trade-offs across model sizes (Section~6.3) \cite{turn0file0}. Moreover, ablation results indicate distinct contributions of the Issue and Evaluation agents, motivating exposure of intermediate configurations as user-selectable compute levels rather than forcing an all-or-nothing scaffold \cite{turn0file0}.

% =========================
% Meta-Agent Router Section
% =========================

\subsection{Meta-Agent Router: Preference-Guided System Selection}
\label{subsec:meta_router}

Our framework supports multiple inference configurations that trade off advice quality against computational cost (token usage).
To expose this trade-off to end users in an interpretable way, we introduce a lightweight \emph{Meta-Agent Router} that maps a
user preference (accuracy vs.\ cost) to one of a fixed set of pipeline configurations. The router is designed to (i) remain
multi-objective in principle, (ii) be monotone in the user preference, and (iii) keep \emph{all} configurations reachable
(i.e., avoid degenerate behavior where one option dominates due to dataset-level averages).

\paragraph{Candidate configurations.}
We assume a fixed, ordered set of $K{+}1$ pipeline configurations
$\mathcal{A} = \{A_0, A_1, \dots, A_K\}$ from cheapest to most expensive under token cost.
In our experiments, we use $K{=}4$ (five choices):
\begin{align*}
A_0 &: \text{Single-LLM (baseline)}\\
A_1 &: \text{Ablation: w/o Issue \& w/o Evaluation}\\
A_2 &: \text{Ablation: w/o Evaluation}\\
A_3 &: \text{Ablation: w/o Issue}\\
A_4 &: \text{Full multi-agent framework.}
\end{align*}
For each $A_i$ we record (from a calibration domain) its mean advice quality $Q_i$ and mean token cost $C_i$.

\paragraph{User preference as a multi-objective scalarization.}
The user specifies nonnegative weights $(w_Q,w_C)$ for quality vs.\ cost. We convert them into a single preference score:
\begin{equation}
p \;=\; \frac{w_Q}{w_Q+w_C} \in [0,1],
\label{eq:p_from_weights}
\end{equation}
where larger $p$ indicates stronger preference for quality (i.e., willingness to spend more tokens).

\paragraph{Why not direct utility maximization over mean $(Q_i,C_i)$?}
A standard approach is to select $\arg\max_i \big(p\widetilde{Q}_i - (1-p)\widetilde{C}_i\big)$ using normalized means.
However, in practice, dataset-level averages can make intermediate configurations appear dominated (e.g., similar quality but
higher token cost), collapsing the router to only one or two options. Since one goal of the router is to provide a stable
and interpretable ``compute knob'' (ensuring that each tier is selectable), we separate (a) the user preference modeling
(Eq.~\ref{eq:p_from_weights}) from (b) the discretization policy that maps $p$ to tiers.

\subsubsection{Cost--Quality Geometry and Near-Uniform Binning}
\label{subsec:bins}

We compute thresholds that are (i) \emph{near-uniform} in $p$ (for interpretability) while (ii) being \emph{aware} of the
empirical cost/quality spacing between configurations. The key idea is to build a one-dimensional progress coordinate over
configurations using both token cost and quality, then blend it with uniform thresholds.

\paragraph{Normalization.}
Let $C_i$ denote mean token cost and $Q_i$ mean quality for configuration $A_i$.
We normalize log-cost and quality to $[0,1]$:
\begin{align}
x_i &= \frac{\log C_i - \log C_0}{\log C_K - \log C_0}, \qquad x_i \in [0,1], \label{eq:log_cost_norm}\\
y_i &= \frac{Q_i - \min_j Q_j}{\max_j Q_j - \min_j Q_j}, \qquad y_i \in [0,1]. \label{eq:quality_norm}
\end{align}
We use $\log C_i$ because token costs are naturally multiplicative (large jumps between tiers), and log-scale yields additive
distances commonly used in systems-style analyses.

\paragraph{Quality+cost progress coordinate (arc-length).}
Define a polygonal chain over the ordered configurations in the $(x,y)$ plane, and compute cumulative arc-length:
\begin{equation}
s_0 = 0, \qquad
s_i = s_{i-1} + \sqrt{(x_i-x_{i-1})^2 + (y_i-y_{i-1})^2}\quad \text{for } i=1,\dots,K.
\label{eq:arc_length}
\end{equation}
Normalize to $[0,1]$:
\begin{equation}
S_i = \frac{s_i}{s_K}\in[0,1].
\label{eq:S_norm}
\end{equation}

\paragraph{Cost--quality midpoints.}
We compute midpoint thresholds between adjacent configurations in this progress coordinate:
\begin{equation}
m_i = \frac{S_{i-1}+S_i}{2}, \qquad i=1,\dots,K.
\label{eq:midpoints_m}
\end{equation}
If used directly, $\{m_i\}$ yields fully cost/quality-aware but potentially non-uniform bins in $p$.

\paragraph{Near-uniform blending.}
Uniform thresholds for $K{+}1$ choices are:
\begin{equation}
u_i = \frac{i}{K+1}, \qquad i=1,\dots,K.
\label{eq:uniform_thresholds}
\end{equation}
We define blended thresholds:
\begin{equation}
b_i(\varepsilon) = (1-\varepsilon)\,u_i + \varepsilon\,m_i, \qquad \varepsilon \in [0,1],
\label{eq:blended_thresholds}
\end{equation}
where $\varepsilon$ controls the trade-off:
$\varepsilon{=}0$ yields exactly uniform bins, and $\varepsilon{=}1$ yields fully cost/quality-aware bins.
In practice we set $\varepsilon \in [0.2,0.4]$ to obtain ``almost-uniform'' bins while respecting the empirical spacing.

\paragraph{Routing rule.}
Let $b_0=0$ and $b_{K+1}=1$. The router selects configuration index
\begin{equation}
j = \sum_{i=1}^{K} \mathbf{1}\!\left[p \ge b_i(\varepsilon)\right],
\qquad \text{and returns } A_j.
\label{eq:routing_rule}
\end{equation}
This rule is monotone in $p$ and guarantees all $K{+}1$ configurations are reachable.

\paragraph{Monotonicity and coverage (sketch).}
Since $\{u_i\}$ is strictly increasing and $\{m_i\}$ is strictly increasing when $C_0<\cdots<C_K$ and the configurations are ordered,
their convex combination $\{b_i(\varepsilon)\}$ is strictly increasing for any $\varepsilon\in[0,1]$. Therefore
$0=b_0<b_1<\cdots<b_K<b_{K+1}=1$ and each interval $[b_j,b_{j+1})$ has positive length, implying every $A_j$ is selected for some user preference.

\subsubsection{Automotive Calibration: Concrete Threshold Values}
\label{subsec:automotive_thresholds}

We compute thresholds once using the Automotive domain (tokens-only) and then apply them unchanged to other domains.
Table~\ref{tab:auto_cost_quality} lists the calibration statistics for the five configurations.

\begin{table}[t]
\centering
\small
\begin{tabular}{lrr}
\toprule
Configuration & Quality $Q_i$ & Tokens $C_i$ \\
\midrule
$A_0$ (Single LLM) & 93.1 & 4{,}822 \\
$A_1$ (w/o Issue \& Eval) & 95.2 & 30{,}045 \\
$A_2$ (w/o Eval) & 94.4 & 30{,}166 \\
$A_3$ (w/o Issue) & 95.0 & 71{,}737 \\
$A_4$ (Full) & 95.2 & 114{,}441 \\
\bottomrule
\end{tabular}
\caption{Automotive calibration statistics (mean quality and mean token cost) used to compute router thresholds.
We use tokens-only cost for binning.}
\label{tab:auto_cost_quality}
\end{table}

Using Eqs.~\ref{eq:log_cost_norm}--\ref{eq:midpoints_m}, the resulting midpoints in the cost--quality progress coordinate are:
\begin{equation}
m \approx [0.2741,\; 0.6385,\; 0.8228,\; 0.9583].
\label{eq:auto_midpoints}
\end{equation}
With $\varepsilon{=}0.3$ in Eq.~\ref{eq:blended_thresholds} (our default ``almost-uniform'' choice),
the blended thresholds are:
\begin{equation}
b(\varepsilon{=}0.3)\approx [0.2222,\; 0.4716,\; 0.6668,\; 0.8475].
\label{eq:auto_thresholds_eps03}
\end{equation}
Therefore, the final bins over $p$ are:
\begin{align*}
p \in [0,0.2222) &\Rightarrow A_0 \\
p \in [0.2222,0.4716) &\Rightarrow A_1 \\
p \in [0.4716,0.6668) &\Rightarrow A_2 \\
p \in [0.6668,0.8475) &\Rightarrow A_3 \\
p \in [0.8475,1] &\Rightarrow A_4.
\end{align*}

\paragraph{Is Automotive-only calibration acceptable?}
Yes, provided it is framed as \emph{threshold calibration on a development split}:
we calibrate thresholds once on Automotive and then \emph{freeze} them for evaluation on other domains.
This avoids per-domain tuning while keeping the router deterministic and reproducible.

\subsubsection{Nested Selection for Backbone Tiers (Single-LLM and Full Framework)}
\label{subsec:nested_tiers}

Some configurations admit meaningful backbone variation.
In particular, our single-LLM baseline supports three backbones (Llama, DeepSeek, GPT-OSS). When the router selects $A_0$, we apply the same binning mechanism
(Eqs.~\ref{eq:log_cost_norm}--\ref{eq:routing_rule}) over the three single-LLM options using their Automotive $(Q,C)$ statistics.
With $\varepsilon{=}0.3$, the resulting two thresholds are:
\begin{equation}
b^{(A_0)}(\varepsilon{=}0.3)\approx [0.3017,\; 0.6851],
\label{eq:single_llm_thresholds}
\end{equation}
yielding:
\begin{align*}
p \in [0,0.3017) &\Rightarrow \text{Llama},\\
p \in [0.3017,0.6851) &\Rightarrow \text{DeepSeek},\\
p \in [0.6851,1] &\Rightarrow \text{GPT-OSS}.
\end{align*}
Analogously, if the full framework admits multiple tiers (e.g., Big vs.\ Medium), we can apply the same nested routing procedure
using the corresponding $(Q,C)$ calibration values.

\subsubsection{Meta-Agent Router Algorithm}
\label{subsec:router_algorithm}

\begin{algorithm}[t]
\caption{Meta-Agent Router (tokens-only, near-uniform cost--quality bins)}
\label{alg:meta_router}
\small
\begin{algorithmic}[1]
\Require User weights $(w_Q,w_C)$; calibration stats $\{(Q_i,C_i)\}_{i=0}^{K}$; blend parameter $\varepsilon$
\State Compute preference $p \leftarrow \frac{w_Q}{w_Q+w_C}$ \Comment{Eq.~\ref{eq:p_from_weights}}
\State Compute $x_i$ and $y_i$ for all $i$ \Comment{Eqs.~\ref{eq:log_cost_norm}, \ref{eq:quality_norm}}
\State Compute $S_i$ via arc-length \Comment{Eqs.~\ref{eq:arc_length}, \ref{eq:S_norm}}
\State Compute midpoints $m_i \leftarrow (S_{i-1}+S_i)/2$ \Comment{Eq.~\ref{eq:midpoints_m}}
\State Compute thresholds $b_i(\varepsilon)\leftarrow (1-\varepsilon)\frac{i}{K+1}+\varepsilon m_i$ \Comment{Eq.~\ref{eq:blended_thresholds}}
\State Select $j \leftarrow \sum_{i=1}^{K}\mathbf{1}[p \ge b_i(\varepsilon)]$ \Comment{Eq.~\ref{eq:routing_rule}}
\State \Return Configuration $A_j$
\end{algorithmic}
\end{algorithm}



% --------------------------- Meta-Agent Routing (Paper-ready) ---------------------------
% --------------------------- Meta-Agent Routing (Paper-ready) ---------------------------
\subsection{Meta-Agent for Preference-Aware System Routing}
\label{sec:meta_agent}

Our framework can be instantiated with multiple configurations that trade off
(i) recommendation quality and (ii) inference cost. As discussed in our cost--quality analysis
(\S6.3) and ablation results (Appendix~C), different agentic components and backbone choices
yield comparable mean quality in some settings while incurring materially different token budgets.
To provide a simple and transparent deployment control, we introduce a \emph{meta-agent} that
routes each user request to an appropriate configuration based on a user-specified preference
between accuracy and cost. This meta-agent does not alter the underlying pipeline; instead, it
implements a lightweight \emph{preference-to-configuration} mapping that keeps all intended
compute tiers reachable and interpretable. \cite{ } % (Add relevant citations if needed.)

\paragraph{User preference score.}
The user specifies nonnegative weights $(w_Q, w_C)$ indicating relative emphasis on quality
and cost. We convert these into a single scalar preference
\begin{equation}
p \;=\; \frac{w_Q}{w_Q+w_C} \in [0,1],
\label{eq:pref_score}
\end{equation}
where larger $p$ indicates greater willingness to spend tokens to improve output quality.

\paragraph{Candidate configurations and token costs.}
Let $\{A_0,\dots,A_4\}$ denote an ordered set of five pipeline configurations from cheapest to
most expensive, with measured token costs $C_0 < C_1 < C_2 < C_3 < C_4$ (tokens-only).
Concretely, we use:
\begin{itemize}
    \item $A_0$: Single-LLM inference (one-prompt, no framework),
    \item $A_1$: Framework w/o Issue Agent and w/o Evaluation Agent,
    \item $A_2$: Framework w/o Evaluation Agent,
    \item $A_3$: Framework w/o Issue Agent,
    \item $A_4$: Full multi-agent framework (Issue + Recommendation + Evaluation + Ranking).
\end{itemize}
This ordering matches the incremental inclusion of agentic components observed in the ablation
study (Appendix~C) and is aligned with the pipeline structure (Figure~2).  % See main paper.

\paragraph{Motivation: why not use utility-optimal thresholds directly?}
A standard approach would select $A_j$ via an argmax of a scalarized utility
(e.g., $p\widetilde{Q}_j - (1-p)\widetilde{C}_j$). However, using mean quality scores alone can
cause intermediate configurations to become \emph{dominated} (never selected) when quality
differences are small relative to token costs. In practical deployments, teams often require
explicit, stable ``gears'' for budgeting, latency/cost envelopes, and operational policy
(including the ability to intentionally choose intermediate tiers). Therefore, we separate:
(i) preference elicitation (Eq.~\ref{eq:pref_score}) from (ii) a calibrated discretization that
ensures near-uniform coverage while still reflecting non-uniform token gaps.

\paragraph{Cost-aware uniformization via log-token geometry.}
Token costs are typically separated by multiplicative factors rather than additive increments.
We therefore define a normalized log-cost coordinate:
\begin{equation}
g_i \;=\; \frac{\log C_i - \log C_0}{\log C_4 - \log C_0},
\qquad i\in\{0,\dots,4\},
\label{eq:log_cost_coord}
\end{equation}
so that $g_0=0$ and $g_4=1$. Next, define cost-aware midpoints between adjacent configurations:
\begin{equation}
m_i \;=\; \frac{g_{i-1}+g_i}{2},
\qquad i\in\{1,\dots,4\}.
\label{eq:midpoints}
\end{equation}
If we used $\{m_i\}$ directly as thresholds, bins would be fully cost-aware but not uniform. For
a more interpretable control (approximately equal probability mass across the preference axis),
we blend these midpoints with uniform thresholds:
\begin{equation}
u_i \;=\; \frac{i}{5}\quad (i=1,\dots,4),
\qquad
b_i(\varepsilon) \;=\; (1-\varepsilon)u_i + \varepsilon m_i,
\qquad \varepsilon\in[0,1].
\label{eq:blended_thresholds}
\end{equation}
Here, $\varepsilon$ controls the trade-off between interpretability and cost-awareness:
$\varepsilon=0$ yields exactly uniform bins, while $\varepsilon=1$ yields purely cost-aware
(midpoint) bins. We use a small $\varepsilon$ (e.g., $0.2$--$0.4$) to obtain \emph{almost-uniform}
bins that still acknowledge large token jumps (notably from $A_0$ to $A_1$).

\paragraph{Routing rule.}
Let $b_0=0$ and $b_5=1$. The meta-agent selects the configuration index $j\in\{0,\dots,4\}$ by
\begin{equation}
j \;=\; \sum_{i=1}^{4} \mathbf{1}\!\left[p \ge b_i(\varepsilon)\right],
\qquad
A \leftarrow A_j,
\label{eq:routing_rule}
\end{equation}
which deterministically maps $p$ to exactly one of the five tiers.

\paragraph{Monotonicity and coverage.}
Assuming $C_0<\cdots<C_4$, the sequence $\{g_i\}$ is strictly increasing and so are the
midpoints $\{m_i\}$. Since $\{u_i\}$ is also strictly increasing, the blended thresholds
$\{b_i(\varepsilon)\}$ are strictly increasing for any $\varepsilon\in[0,1]$. Hence each interval
$[b_j, b_{j+1})$ has positive length, guaranteeing that every configuration $A_j$ is selected for
a non-empty range of $p$. This provides stable user control while remaining consistent with
token-cost geometry.

\paragraph{Example: token-only thresholds for the automotive setting.}
Using the measured token costs (tokens-only):
\begin{equation}
(C_0,C_1,C_2,C_3,C_4)
=
(4822,\;30045,\;30166,\;71737,\;114441),
\label{eq:example_costs}
\end{equation}
we compute $g_i$ from Eq.~\ref{eq:log_cost_coord}, then $m_i$ from Eq.~\ref{eq:midpoints}, and
finally the blended thresholds from Eq.~\ref{eq:blended_thresholds}. For $\varepsilon=0.3$,
this yields:
\begin{equation}
\left(b_1,b_2,b_3,b_4\right)
\approx
(0.2267,\;0.4535,\;0.6347,\;0.8379).
\label{eq:example_thresholds}
\end{equation}
Thus, the five routing bins are:
\begin{align}
p &\in [0,\,0.2267) &&\Rightarrow\; A_0 \quad \text{(Single LLM)}, \nonumber\\
p &\in [0.2267,\,0.4535) &&\Rightarrow\; A_1 \quad \text{(w/o Issue \& Eval)}, \nonumber\\
p &\in [0.4535,\,0.6347) &&\Rightarrow\; A_2 \quad \text{(w/o Eval)}, \nonumber\\
p &\in [0.6347,\,0.8379) &&\Rightarrow\; A_3 \quad \text{(w/o Issue)}, \nonumber\\
p &\in [0.8379,\,1] &&\Rightarrow\; A_4 \quad \text{(Full framework)}.
\label{eq:bins}
\end{align}

\paragraph{Backbone selection within tiers.}
Some tiers admit multiple backbone choices. In particular, $A_0$ (single-LLM inference) can use
any of $\{\textsc{Llama}, \textsc{GPT-OSS}, \textsc{DeepSeek}\}$, consistent with our single-model
baseline evaluation (Table~1). We implement backbone selection as a second-stage choice that is
invoked only when needed:
\begin{equation}
M =
\begin{cases}
\{\textsc{Llama}, \textsc{GPT-OSS}, \textsc{DeepSeek}\}, & \text{if } A=A_0,\\
\{\textsc{Big}, \textsc{Medium}\}, & \text{if } A=A_4 \text{ and multiple tiers are enabled},\\
\varnothing, & \text{otherwise.}
\end{cases}
\label{eq:conditional_backbone}
\end{equation}
In deployments that require a single deterministic backbone per tier, one may fix the backbone
(e.g., GPT-OSS for $A_0$) and retain only the pipeline-level routing of Eq.~\ref{eq:routing_rule}.

\paragraph{Discussion.}
The proposed meta-agent provides a simple interface for practitioners to trade off inference cost
and output quality while maintaining interpretable, stable compute tiers. By blending uniform and
cost-aware thresholds, the routing policy yields near-uniform preference bins yet respects the
fact that token budgets are not evenly spaced across pipeline variants. This design is particularly
useful in settings where mean quality differences between variants are modest (as observed in our
cost--quality results) but operational policies require explicit intermediate budget options.
% ---------------------------------------------------------------------------------------
\subsection{Meta Agent}
\label{sec:meta_agent}

Our framework can be instantiated with multiple configurations that trade off
(i) recommendation quality and (ii) inference cost. As discussed in our cost--quality analysis
(\S6.3) and ablation results (Appendix~C), different agentic components and backbone choices
yield comparable mean quality in some settings while incurring materially different token budgets.
To provide a simple and transparent deployment control, we introduce a \emph{meta-agent} that
routes each user request to an appropriate configuration based on a user-specified preference
between accuracy and cost. This meta-agent does not alter the underlying pipeline; instead, it
implements a lightweight \emph{preference-to-configuration} mapping that keeps all intended
compute tiers reachable and interpretable. \cite{ } % (Add relevant citations if needed.)

\paragraph{User preference score.}
The user specifies nonnegative weights $(w_Q, w_C)$ indicating relative emphasis on quality
and cost. We convert these into a single scalar preference
\begin{equation}
p \;=\; \frac{w_Q}{w_Q+w_C} \in [0,1],
\label{eq:pref_score}
\end{equation}
where larger $p$ indicates greater willingness to spend tokens to improve output quality.

\paragraph{Candidate configurations and token costs.}
Let $\{A_0,\dots,A_4\}$ denote an ordered set of five pipeline configurations from cheapest to
most expensive, with measured token costs $C_0 < C_1 < C_2 < C_3 < C_4$ (tokens-only).
Concretely, we use:
\begin{itemize}
    \item $A_0$: Single-LLM inference (one-prompt, no framework),
    \item $A_1$: Framework w/o Issue Agent and w/o Evaluation Agent,
    \item $A_2$: Framework w/o Evaluation Agent,
    \item $A_3$: Framework w/o Issue Agent,
    \item $A_4$: Full multi-agent framework (Issue + Recommendation + Evaluation + Ranking).
\end{itemize}
This ordering matches the incremental inclusion of agentic components observed in the ablation
study (Appendix~C) and is aligned with the pipeline structure (Figure~2).  % See main paper.

\paragraph{Motivation: why not use utility-optimal thresholds directly?}
A standard approach would select $A_j$ via an argmax of a scalarized utility
(e.g., $p\widetilde{Q}_j - (1-p)\widetilde{C}_j$). However, using mean quality scores alone can
cause intermediate configurations to become \emph{dominated} (never selected) when quality
differences are small relative to token costs. In practical deployments, teams often require
explicit, stable ``gears'' for budgeting, latency/cost envelopes, and operational policy
(including the ability to intentionally choose intermediate tiers). Therefore, we separate:
(i) preference elicitation (Eq.~\ref{eq:pref_score}) from (ii) a calibrated discretization that
ensures near-uniform coverage while still reflecting non-uniform token gaps.

\paragraph{Cost-aware uniformization via log-token geometry.}
Token costs are typically separated by multiplicative factors rather than additive increments.
We therefore define a normalized log-cost coordinate:
\begin{equation}
g_i \;=\; \frac{\log C_i - \log C_0}{\log C_4 - \log C_0},
\qquad i\in\{0,\dots,4\},
\label{eq:log_cost_coord}
\end{equation}
so that $g_0=0$ and $g_4=1$. Next, define cost-aware midpoints between adjacent configurations:
\begin{equation}
m_i \;=\; \frac{g_{i-1}+g_i}{2},
\qquad i\in\{1,\dots,4\}.
\label{eq:midpoints}
\end{equation}
If we used $\{m_i\}$ directly as thresholds, bins would be fully cost-aware but not uniform. For
a more interpretable control (approximately equal probability mass across the preference axis),
we blend these midpoints with uniform thresholds:
\begin{equation}
\begin{split}
u_i &= \frac{i}{5}, \quad i \in \{1,2,3,4\},\\
b_i(\varepsilon) &= (1-\varepsilon)\,u_i + \varepsilon\, m_i, \quad \varepsilon \in [0,1].
\end{split}
\label{eq:blended_thresholds}
\end{equation}

Here, $\varepsilon$ controls the trade-off between interpretability and cost-awareness:
$\varepsilon=0$ yields exactly uniform bins, while $\varepsilon=1$ yields purely cost-aware
(midpoint) bins. We use a small $\varepsilon$ (e.g., $0.2$--$0.4$) to obtain \emph{almost-uniform}
bins that still acknowledge large token jumps (notably from $A_0$ to $A_1$).

\paragraph{Routing rule.}
Let $b_0=0$ and $b_5=1$. The meta-agent selects the configuration index $j\in\{0,\dots,4\}$ by
\begin{equation}
j \;=\; \sum_{i=1}^{4} \mathbf{1}\!\left[p \ge b_i(\varepsilon)\right],
\qquad
A \leftarrow A_j,
\label{eq:routing_rule}
\end{equation}
which deterministically maps $p$ to exactly one of the five tiers.

\paragraph{Monotonicity and coverage.}
Assuming $C_0<\cdots<C_4$, the sequence $\{g_i\}$ is strictly increasing and so are the
midpoints $\{m_i\}$. Since $\{u_i\}$ is also strictly increasing, the blended thresholds
$\{b_i(\varepsilon)\}$ are strictly increasing for any $\varepsilon\in[0,1]$. Hence each interval
$[b_j, b_{j+1})$ has positive length, guaranteeing that every configuration $A_j$ is selected for
a non-empty range of $p$. This provides stable user control while remaining consistent with
token-cost geometry.

\paragraph{Example: token-only thresholds for the automotive setting.}
Using the measured token costs (tokens-only):
\begin{table}[ht!]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{c c c c c}
\toprule
$C_0$ & $C_1$ & $C_2$ & $C_3$ & $C_4$ \\
\midrule
4822 & 30045 & 30166 & 71737 & 114441 \\
\bottomrule
\end{tabular}
\caption{Token consumed for the five pipeline configurations for Automotive domain.}
\label{tab:example_costs}
\end{table}


We compute $g_i$ from Eq.~\ref{eq:log_cost_coord}, then $m_i$ from Eq.~\ref{eq:midpoints}, and
finally the blended thresholds from Eq.~\ref{eq:blended_thresholds}. For $\varepsilon=0.3$,
this yields:
\begin{equation}
\left(b_1,b_2,b_3,b_4\right)
\approx
(0.2267,\;0.4535,\;0.6347,\;0.8379).
\label{eq:example_thresholds}
\end{equation}
Thus, the five routing bins are:
\[
\begin{aligned}
p &\in [0,0.2267) &\Rightarrow A_0, \\
p &\in [0.2267,0.4535) &\Rightarrow A_1, \\
p &\in [0.4535,0.6347) &\Rightarrow A_2, \\
p &\in [0.6347,0.8379) &\Rightarrow A_3, \\
p &\in [0.8379,1] &\Rightarrow A_4.
\end{aligned}
\]
These bins are close to uniform (nominally $0.2$ width) while reflecting the large multiplicative jump from $A_0$ to $A_1$ in token cost.
\paragraph{Backbone selection within tiers.}
Some tiers admit multiple backbone choices. In particular, $A_0$ (single-LLM inference) can use
any of $\{\textsc{Llama}, \textsc{DeepSeek}\}$, consistent with our single-model
baseline evaluation (Table~1). We implement backbone selection as a second-stage choice that is
invoked only when needed:
\begin{equation}
M =
\begin{cases}
\{\textsc{Llama}, \textsc{DeepSeek}\}, & \text{if } A=A_0,\\
\{\textsc{Big}, \textsc{Medium}\}, & \text{if } A=A_4 \text{ and multiple tiers are enabled},\\
\varnothing, & \text{otherwise.}
\end{cases}
\label{eq:conditional_backbone}
\end{equation}
In deployments that require a single deterministic backbone per tier, one may fix the backbone
(e.g., GPT-OSS for $A_0$) and retain only the pipeline-level routing of Eq.~\ref{eq:routing_rule}.

\paragraph{Discussion.}
The proposed meta-agent provides a simple interface for practitioners to trade off inference cost
and output quality while maintaining interpretable, stable compute tiers. By blending uniform and
cost-aware thresholds, the routing policy yields near-uniform preference bins yet respects the
fact that token budgets are not evenly spaced across pipeline variants. This design is particularly
useful in settings where mean quality differences between variants are modest (as observed in our
cost--quality results) but operational policies require explicit intermediate budget options.
% ---------------------------------------------------------------------------------------




==> notes.tex <==
Add $\eta$ justification, experiments etc.
Add future work(RAG for policy, )
Human Evaluation, correlation etc
update figure fonts
add token and latency accounting per approach


Remove gpt oss 120 b single model results 
